Generating an Image From 1,000 Words: Enhancing Text-to-Image With Structured Captions

Text-to-image models have rapidly evolved from casual creative tools to professional-grade systems, achieving unprecedented levels of image quality and realism. Yet, most models are trained to map short prompts into detailed images, creating a gap between sparse textual input and rich visual outputs. This mismatch reduces controllability, as models often fill in missing details arbitrarily, biasing toward average user preferences and limiting precision for professional use. We address this limitation by training the first open-source text-to-image model on long structured captions, where every training sample is annotated with the same set of fine-grained attributes. This design maximizes expressive coverage and enables disentangled control over visual factors. To process long captions efficiently, we propose DimFusion, a fusion mechanism that integrates intermediate tokens from a lightweight LLM without increasing token length. We also introduce the Text-as-a-Bottleneck Reconstruction (TaBR) evaluation protocol. By assessing how well real images can be reconstructed through a captioning-generation loop, TaBR directly measures controllability and expressiveness, even for very long captions where existing evaluation methods fail. Finally, we demonstrate our contributions by training the large-scale model FIBO, achieving state-of-the-art prompt alignment among open-source models. Model weights are publicly available at https://huggingface.co/briaai/FIBO

==> Figures/json_vs_short/json_vs_short.tex <==
% Preamble: \usepackage{graphicx,array}
\setlength{\tabcolsep}{0.5pt}
\renewcommand{\arraystretch}{1.0}

\begin{figure}[t]
\centering
\newcommand{\imgw}{0.24\linewidth} % 4 images × 0.24 = 0.96 (safe)
\begin{tabular}{@{}cccc@{}}
  % Header for row 1
  \multicolumn{4}{@{}l@{}}{{\scriptsize\textbf{Long structured captions training}}} \\[-1pt]
  % Row 1 images
  \includegraphics[width=\imgw]{Figures/json_vs_short/images/json_1.jpg} &
  \includegraphics[width=\imgw]{Figures/json_vs_short/images/json_2.jpg} &
  \includegraphics[width=\imgw]{Figures/json_vs_short/images/json_3.jpg} &
  \includegraphics[width=\imgw]{Figures/json_vs_short/images/json_4.jpg} \\[-2pt]
  % Header for row 2
  \multicolumn{4}{@{}l@{}}{{\scriptsize\textbf{Short captions training}}} \\[-1pt]
  % Row 2 images
  \includegraphics[width=\imgw]{Figures/json_vs_short/images/short_1.jpg} &
  \includegraphics[width=\imgw]{Figures/json_vs_short/images/short_2.jpg} &
  \includegraphics[width=\imgw]{Figures/json_vs_short/images/short_3.jpg} &
  \includegraphics[width=\imgw]{Figures/json_vs_short/images/short_4.jpg} \\
\end{tabular}

\vspace{-3pt}
\caption{\textbf{Qualitative comparison between models trained with long structured captions and short captions.} After $100$K training steps, the model trained with long captions produces more coherent and visually detailed images, demonstrating faster convergence and better alignment with the prompt.}
\label{fig:caption-length-comparison}
\end{figure}


==> Figures/teaser/teaser.tex <==

\twocolumn[{
\renewcommand\twocolumn[1][]{#1}

\vspace{-0.8cm}
\maketitle
\begin{center}
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/teaser/teaser.png}
  \vspace{-0.7cm}
  \captionof{figure}{\textbf{A sample from FIBO with its structured JSON description.} Each element in the scene (illustrated here with the Eight of Spades) is described in the JSON, including its position, texture, and relations to neighboring objects. 
  The JSON further specifies global attributes such as background, lighting, composition, and photographic characteristics, providing a complete, structured depiction of the image content.}
  \label{fig:teaser}
\end{center}
}]

==> Figures/user_study/user_study.tex <==

\begin{figure}[t]
\centering


  \includegraphics[width=\linewidth]{Figures/user_study/preference_user_study.jpg}

  \includegraphics[width=\linewidth]{Figures/user_study/tabr_user_study.jpg}


\vspace{-3mm}
\caption{\textbf{User study examples.} 
\textbf{(Top)} and \textbf{(Bottom)} visualizations of the user study conducted for overall preference and TaBR respectively.}
\label{fig:user_study_ui}
\vspace{-2mm}
\end{figure}

==> plots/model_figure.tex <==
\tikzstyle{every node}=[font=\large]
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt , rounded corners = 9.0] (1.25,17.5) rectangle  node {\LARGE Caption} (3.75,16.25);
\draw [ fill={rgb,255:red,202; green,240; blue,254} , line width=0.8pt , rounded corners = 9.0] (0,15.5) rectangle (5,-3.25);
\node [font=\Large] at (2.5,15) {LLM};
\draw [line width=0.8pt, ->, >=Stealth] (2.5,16.25) -- (2.5,15.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (3.75,14.25) rectangle (4.25,13.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (0.75,14.25) rectangle (1.25,13.75);
\node [font=\Large] at (-3.5,12.75) {};
\node [font=\Large] at (-3.5,12.75) {};
\node [font=\Large] at (-4.25,12.75) {};
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (1.75,14.25) rectangle (2.25,13.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (2.75,14.25) rectangle (3.25,13.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (0.25,13.25) rectangle  node {\large LLM Block} (4.75,12.75);
\draw [line width=0.8pt, ->, >=Stealth] (2.5,13.75) -- (2.5,13.25);
\node [font=\Huge] at (3,13) {};
\node [font=\Huge] at (3,13) {};
\node [font=\Huge] at (3,13) {};
\draw [line width=0.8pt, ->, >=Stealth] (2.5,12.75) -- (2.5,12.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (3.75,12.25) rectangle (4.25,11.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (0.75,12.25) rectangle (1.25,11.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (1.75,12.25) rectangle (2.25,11.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (2.75,12.25) rectangle (3.25,11.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (0.25,8.75) rectangle  node {\large LLM Block} (4.75,8.25);
\draw [line width=0.8pt, ->, >=Stealth] (2.5,11.5) -- (2.5,8.75);
\node [font=\Huge] at (3,8.5) {};
\node [font=\Huge] at (3,8.5) {};
\node [font=\Huge] at (3,8.5) {};
\draw [line width=0.8pt, ->, >=Stealth] (2.5,8.25) -- (2.5,7.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (3.75,7.75) rectangle (4.25,7.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (0.75,7.75) rectangle (1.25,7.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (1.75,7.75) rectangle (2.25,7.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (2.75,7.75) rectangle (3.25,7.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (0.25,4) rectangle  node {\large LLM Block} (4.75,3.5);
\draw [line width=0.8pt, ->, >=Stealth] (2.5,6.5) -- (2.5,4);
\node [font=\Huge] at (3,3.75) {};
\node [font=\Huge] at (3,3.75) {};
\node [font=\Huge] at (3,3.75) {};
\draw [line width=0.8pt, ->, >=Stealth] (2.5,3.5) -- (2.5,3);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (3.75,2.75) rectangle (4.25,2.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (0.75,2.75) rectangle (1.25,2.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (1.75,2.75) rectangle (2.25,2.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (2.75,2.75) rectangle (3.25,2.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (0.25,-0.5) rectangle  node {\large LLM Block} (4.75,-1);
\draw [line width=0.8pt, ->, >=Stealth] (2.5,2.25) -- (2.5,-0.5);
\node [font=\Huge] at (3,-0.75) {};
\node [font=\Huge] at (3,-0.75) {};
\node [font=\Huge] at (3,-0.75) {};
\draw [line width=0.8pt, ->, >=Stealth] (5,12) -- (6.25,12);
\draw [line width=0.8pt, ->, >=Stealth] (5,-1.75) -- (6.25,-1.75);
\draw [line width=0.8pt, ->, >=Stealth] (5,7.5) -- (6.25,7.5);
\draw [line width=0.8pt, ->, >=Stealth] (2.5,-1) -- (2.5,-1.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (3.75,-1.5) rectangle (4.25,-2);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (0.75,-1.5) rectangle (1.25,-2);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (1.75,-1.5) rectangle (2.25,-2);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (2.75,-1.5) rectangle (3.25,-2);
\draw [line width=0.8pt, ->, >=Stealth] (5,2.5) -- (6.25,2.5);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,13.75) rectangle (13.75,13.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,13.75) rectangle (10.75,13.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,13.75) rectangle (11.75,13.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,13.75) rectangle (12.75,13.25);
\draw [line width=0.8pt, ->, >=Stealth] (12,11.75) -- (12,11);
\draw [ fill={rgb,255:red,202; green,240; blue,254} , line width=0.8pt , rounded corners = 9.0] (14.25,17.25) rectangle  node {\Large Noisy Latents} (18,16);
\draw [ fill={rgb,255:red,0; green,253; blue,255} , line width=0.8pt , rounded corners = 9.0] (14.25,15.5) rectangle  node {\Large Linear} (18,14.25);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (17.25,12.25) rectangle (17.75,11.75);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (14.25,12.25) rectangle (14.75,11.75);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (15.25,12.25) rectangle (15.75,11.75);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (16.25,12.25) rectangle (16.75,11.75);
\draw [line width=0.8pt, ->, >=Stealth] (16,11.75) -- (16,11);
\draw [ fill={rgb,255:red,0; green,253; blue,255} , line width=0.8pt , rounded corners = 9.0] (6.25,12.5) rectangle  node {\Large Linear} (8,11.25);
\draw [ fill={rgb,255:red,0; green,253; blue,255} , line width=0.8pt , rounded corners = 9.0] (6.25,-1.25) rectangle  node {\Large Linear} (8,-2.5);
\draw [ fill={rgb,255:red,0; green,253; blue,255} , line width=0.8pt , rounded corners = 9.0] (6.25,8) rectangle  node {\Large Linear} (8,6.75);
\draw [ fill={rgb,255:red,0; green,253; blue,255} , line width=0.8pt , rounded corners = 9.0] (6.25,3) rectangle  node {\Large Linear} (8,1.75);
\draw [ fill={rgb,255:red,204; green,232; blue,181} , line width=0.8pt ] (10,11) rectangle  node {\Large Double-Stream Block} (17.75,10.5);
\draw [ fill={rgb,255:red,204; green,232; blue,181} , line width=0.8pt ] (10,6.75) rectangle  node {\Large Double-Stream Block} (17.75,6.25);
\draw [ fill={rgb,255:red,204; green,232; blue,181} , line width=0.8pt ] (10,1.75) rectangle  node {\Large Single-Stream Block} (17.75,1.25);
\draw [ fill={rgb,255:red,204; green,232; blue,181} , line width=0.8pt ] (10,-2.5) rectangle  node {\Large Single-Stream Block} (17.75,-3);
\draw [line width=0.8pt, ->, >=Stealth] (8,12) -- (10,12);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (10.25,12.25) rectangle (10.75,11.75);
\node [font=\Large] at (11.25,13) {};
\node [font=\Large] at (11.25,13) {};
\node [font=\Large] at (11.25,13) {};
\node [font=\Large] at (11.25,13) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,12.25) rectangle (10.75,11.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (11.25,12.25) rectangle (11.75,11.75);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,12.25) rectangle (11.75,11.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (12.25,12.25) rectangle (12.75,11.75);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,12.25) rectangle (12.75,11.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (13.25,12.25) rectangle (13.75,11.75);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,12.25) rectangle (13.75,11.75);
\draw [line width=0.8pt, ->, >=Stealth] (12,13.25) -- (12,12.25);
\draw [line width=0.8pt, ->, >=Stealth] (16,16) -- (16,15.5);
\draw [line width=0.8pt, ->, >=Stealth] (16,14.25) -- (16,12.25);
\draw [line width=0.8pt, ->, >=Stealth] (12,9.5) -- (12,9);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (17.5,10) rectangle (18,9.5);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (15.25,10) rectangle (15.75,9.5);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (14.25,10) rectangle (14.75,9.5);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (16.25,10) rectangle (16.75,9.5);
\draw [line width=0.8pt, ->, >=Stealth] (16,9.5) -- (16,6.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (10.25,10) rectangle (10.75,9.5);
\node [font=\Large] at (11.25,10.25) {};
\node [font=\Large] at (11.25,10.25) {};
\node [font=\Large] at (11.25,10.25) {};
\node [font=\Large] at (11.25,10.25) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,10) rectangle (10.75,9.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (11.25,10) rectangle (11.75,9.5);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,10) rectangle (11.75,9.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (12.25,10) rectangle (12.75,9.5);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,10) rectangle (12.75,9.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (13.25,10) rectangle (13.75,9.5);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,10) rectangle (13.75,9.5);
\draw [line width=0.8pt, ->, >=Stealth] (12,10.5) -- (12,10);
\draw [line width=0.8pt, ->, >=Stealth] (16,10.5) -- (16,10);
\node [font=\Large] at (14.25,8.75) {};
\node [font=\Large] at (14.25,8.75) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,9) rectangle (13.75,8.5);
\node [font=\Large] at (14.5,8.25) {};
\node [font=\Large] at (14.75,8.25) {};
\node [font=\Large] at (14.25,7.5) {};
\node [font=\Large] at (14.25,8.75) {};
\node [font=\Large] at (14.25,8.75) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,9) rectangle (12.75,8.5);
\node [font=\Large] at (13.25,7.5) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,9) rectangle (11.75,8.5);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,9) rectangle (10.75,8.5);
\draw [line width=0.8pt, ->, >=Stealth] (8,7.5) -- (10,7.5);
\node [font=\Huge] at (12.5,8.75) {};
\node [font=\Huge] at (12.5,8.75) {};
\draw [line width=0.8pt, ->, >=Stealth] (12,8.5) -- (12,8);
\draw [line width=0.8pt, ->, >=Stealth] (12,7.25) -- (12,6.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (10.25,7.75) rectangle (10.75,7.25);
\node [font=\Large] at (11.25,8) {};
\node [font=\Large] at (11.25,8) {};
\node [font=\Large] at (11.25,8) {};
\node [font=\Large] at (11.25,8) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,7.75) rectangle (10.75,7.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (11.25,7.75) rectangle (11.75,7.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,7.75) rectangle (11.75,7.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (12.25,7.75) rectangle (12.75,7.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,7.75) rectangle (12.75,7.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (13.25,7.75) rectangle (13.75,7.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,7.75) rectangle (13.75,7.25);
\draw [line width=0.8pt, ->, >=Stealth] (12,4.5) -- (12,4);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (17.25,5) rectangle (17.75,4.5);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (14.25,5) rectangle (14.75,4.5);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (15.25,5) rectangle (15.75,4.5);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (16.25,5) rectangle (16.75,4.5);
\draw [line width=0.8pt, ->, >=Stealth] (16,4.5) -- (16,1.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (10.25,5) rectangle (10.75,4.5);
\node [font=\Large] at (11.25,6) {};
\node [font=\Large] at (11.25,6) {};
\node [font=\Large] at (11.25,6) {};
\node [font=\Large] at (11.25,6) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,5) rectangle (10.75,4.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (11.25,5) rectangle (11.75,4.5);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,5) rectangle (11.75,4.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (12.25,5) rectangle (12.75,4.5);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,5) rectangle (12.75,4.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (13.25,5) rectangle (13.75,4.5);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,5) rectangle (13.75,4.5);
\draw [line width=0.8pt, ->, >=Stealth] (12,6.25) -- (12,5.75);
\draw [line width=0.8pt, ->, >=Stealth] (16,6.25) -- (16,5.75);
\node [font=\Large] at (14.25,3.75) {};
\node [font=\Large] at (14.25,3.75) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,4) rectangle (13.75,3.5);
\node [font=\Large] at (14.5,3.25) {};
\node [font=\Large] at (14.75,3.25) {};
\node [font=\Large] at (14.25,2.5) {};
\node [font=\Large] at (14.25,3.75) {};
\node [font=\Large] at (14.25,3.75) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,4) rectangle (12.75,3.5);
\node [font=\Large] at (13.25,2.5) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,4) rectangle (11.75,3.5);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,4) rectangle (10.75,3.5);
\node [font=\Huge] at (12.5,3.75) {};
\node [font=\Huge] at (12.5,3.75) {};
\draw [line width=0.8pt, ->, >=Stealth] (12,3.5) -- (12,3);
\draw [line width=0.8pt, ->, >=Stealth] (12,2.25) -- (12,1.75);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (10.25,2.75) rectangle (10.75,2.25);
\node [font=\Large] at (11.25,3) {};
\node [font=\Large] at (11.25,3) {};
\node [font=\Large] at (11.25,3) {};
\node [font=\Large] at (11.25,3) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,2.75) rectangle (10.75,2.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (11.25,2.75) rectangle (11.75,2.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,2.75) rectangle (11.75,2.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (12.25,2.75) rectangle (12.75,2.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,2.75) rectangle (12.75,2.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (13.25,2.75) rectangle (13.75,2.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,2.75) rectangle (13.75,2.25);
\draw [line width=0.8pt, ->, >=Stealth] (12,0.25) -- (12,-0.25);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (17.25,0.75) rectangle (17.75,0.25);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (14.25,0.75) rectangle (14.75,0.25);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (15.25,0.75) rectangle (15.75,0.25);
\draw [ fill={rgb,255:red,211; green,87; blue,254} , line width=0.8pt ] (16.25,0.75) rectangle (16.75,0.25);
\draw [line width=0.8pt, ->, >=Stealth] (16,0.25) -- (16,-2.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (10.25,0.75) rectangle (10.75,0.25);
\node [font=\Large] at (11.25,1) {};
\node [font=\Large] at (11.25,1) {};
\node [font=\Large] at (11.25,1) {};
\node [font=\Large] at (11.25,1) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,0.75) rectangle (10.75,0.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (11.25,0.75) rectangle (11.75,0.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,0.75) rectangle (11.75,0.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (12.25,0.75) rectangle (12.75,0.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,0.75) rectangle (12.75,0.25);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (13.25,0.75) rectangle (13.75,0.25);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,0.75) rectangle (13.75,0.25);
\draw [line width=0.8pt, ->, >=Stealth] (12,1.25) -- (12,0.75);
\draw [line width=0.8pt, ->, >=Stealth] (16,1.25) -- (16,0.75);
\node [font=\Large] at (14,-0.5) {};
\node [font=\Large] at (14,-0.5) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,-0.25) rectangle (13.75,-0.75);
\node [font=\Large] at (14.25,-1) {};
\node [font=\Large] at (14.5,-1) {};
\node [font=\Large] at (14,-1.75) {};
\node [font=\Large] at (14,-0.5) {};
\node [font=\Large] at (14,-0.5) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,-0.25) rectangle (12.75,-0.75);
\node [font=\Large] at (13.25,-1.75) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,-0.25) rectangle (11.75,-0.75);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,-0.25) rectangle (10.75,-0.75);
\node [font=\Huge] at (12.5,-0.5) {};
\node [font=\Huge] at (12.5,-0.5) {};
\draw [line width=0.8pt, ->, >=Stealth] (12,-0.75) -- (12,-1.25);
\draw [line width=0.8pt, ->, >=Stealth] (12,-2) -- (12,-2.5);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (10.25,-1.5) rectangle (10.75,-2);
\node [font=\Large] at (11.25,-1.25) {};
\node [font=\Large] at (11.25,-1.25) {};
\node [font=\Large] at (11.25,-1.25) {};
\node [font=\Large] at (11.25,-1.25) {};
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (10.5,-1.5) rectangle (10.75,-2);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (11.25,-1.5) rectangle (11.75,-2);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (11.5,-1.5) rectangle (11.75,-2);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (12.25,-1.5) rectangle (12.75,-2);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (12.5,-1.5) rectangle (12.75,-2);
\draw [ fill={rgb,255:red,224; green,237; blue,212} , line width=0.8pt ] (13.25,-1.5) rectangle (13.75,-2);
\draw [ fill={rgb,255:red,255; green,140; blue,130} , line width=0.8pt ] (13.5,-1.5) rectangle (13.75,-2);
\draw [line width=0.8pt, ->, >=Stealth] (8,2.5) -- (10,2.5);
\draw [line width=0.8pt, ->, >=Stealth] (8,-1.75) -- (10,-1.75);
\draw [ fill={rgb,255:red,0; green,253; blue,255} , line width=0.8pt , rounded corners = 9.0] (14.25,-3.75) rectangle  node {\Large Linear} (18,-5);
\draw [line width=0.8pt, ->, >=Stealth] (16,-3) -- (16,-3.75);
\draw [line width=0.8pt, ->, >=Stealth] (16,-5) -- (16,-5.75);
\draw [ fill={rgb,255:red,202; green,240; blue,254} , line width=0.8pt , rounded corners = 9.0] (14.25,-5.75) rectangle  node {\Large Output} (18,-7);
\node [font=\Large] at (12,1.75) {};
\node [font=\Large] at (12,1.5) {};
\node [font=\Large] at (2.5,2.75) {};
\node [font=\Large] at (2.5,2.5) {};
\node [font=\Large] at (-2,2.75) {};
\node [font=\Large] at (2.5,2.5) {};
\node [font=\Large] at (16,1.75) {};
\node [font=\Large] at (18,2.5) {};
\node [font=\Large] at (18,2.5) {};
\node [font=\Large] at (18.5,2) {};
\node [font=\LARGE] at (2.5,7) {};
\node [font=\LARGE] at (2.5,7.25) {};
\node [font=\LARGE] at (2.5,7.5) {$.$};
\node [font=\LARGE] at (2.5,7.25) {$.$};
\node [font=\LARGE] at (2.5,7) {$.$};
\node [font=\Large] at (12,5.5) {.};
\node [font=\Large] at (12,5.25) {.};
\node [font=\Large] at (12,5.75) {.};
\node [font=\Large] at (12.5,5) {};
\node [font=\Large] at (16,5.5) {.};
\node [font=\Large] at (16,5.75) {.};
\node [font=\Large] at (16,5.25) {.};
\node [font=\Large] at (16.75,-4.75) {};
\draw [ fill={rgb,255:red,0; green,253; blue,255} , line width=0.8pt , rounded corners = 9.0] (9.25,15.5) rectangle  node {\Large Linear} (14,14.25);
\node at (5.5,-1.75) [circ] {};
\draw[domain=-14:-14,samples=100,smooth] plot (\x,{1*sin(1*\x r +14 r ) +1.25});
\draw [short] (5.5,-1.75) -- (5.5,16.75);
\draw [->, >=Stealth] (12,14.25) -- (12,13.75);




\draw (5.5,16.75) to[short] (12,16.75);
\draw [->, >=Stealth] (12,16.75) -- (12,15.5);


==> tables/dimfusion_fid_compariosn.tex <==
\begin{table}[t]
\centering
{\setlength{\tabcolsep}{8pt}
\begin{tabular}{lc}
\toprule
\textbf{Architecture} & \textbf{FID} ↓ \\
\midrule
T5 & 36.46 \\
TokenFusion & 15.9 \\
DimFusion & \textbf{15.58}\\
\bottomrule 
\end{tabular}
}
\caption{\textbf{FID comparison between different architectures.} We report the FID on 30K images from the COCO-2014 validation split~\cite{lin2014microsoft}. Both fusion strategies substantially outperform the T5 baseline, with DimFusion achieving the best FID.}
\label{tab:dimfusion-fid-comparison}
\end{table}

